Dream to Manipulate: Compositional World Models Empowering Robot Imitation Learning with Imagination

A world model provides an agent with a representation of its environment, enabling it to predict the causal consequences of its actions. Current world models typically cannot directly and explicitly imitate the actual environment in front of a robot, often resulting in unrealistic behaviors and hallucinations that make them unsuitable for real-world robotics applications. To overcome those challenges, we propose to rethink robot world models as learnable digital twins. We introduce DreMa, a new approach for constructing digital twins automatically using learned explicit representations of the real world and its dynamics, bridging the gap between traditional digital twins and world models. DreMa replicates the observed world and its structure by integrating Gaussian Splatting and physics simulators, allowing robots to imagine novel configurations of objects and to predict the future consequences of robot actions thanks to its compositionality. We leverage this capability to generate new data for imitation learning by applying equivariant transformations to a small set of demonstrations. Our evaluations across various settings demonstrate significant improvements in accuracy and robustness by incrementing actions and object distributions, reducing the data needed to learn a policy and improving the generalization of the agents. As a highlight, we show that a real Franka Emika Panda robot, powered by DreMa's imagination, can successfully learn novel physical tasks from just a single example per task variation (one-shot policy learning). Our project page can be found in: https://dreamtomanipulate.github.io/.

==> text/old_text/data_augmentation_old.tex <==
\section{Equivariant augmentation for Imitation Learning}

\begin{figure}
\centering
\includegraphics[width=\textwidth]{images/augmentation_visualization.png} \\
\caption{Visualization of the augmentations proposed. From left to right: the original trajectory and environment, the translation augmentation, rotation augmentation, and rotation of trajectory augmentation. }
\label{fig:augmentation_vis}
\end{figure}


The world model should be able to execute the robot's actions in imagination, meaning that $\mathbf{A}$ can be executed inside the simulation. This feature is exploited to check the causal consequence to the objects and to store the final position $g$ reached by the objects. These positions are used to check the data generated by the world model is capable of solving the task. 

The physics-powered world model is used to create a synthetic set $\mathcal{D}_{aug}$ by imposing that the robot's actions $\mathbf{A}$ are equivariant to any rigid transformation of the environment that allows the objects to reach the goal $g$. We propose two equivariant augmentations for the robot actions: roto-translation of environment and objects and rotations of the objects. In ~\Fig{fig:augmentation_vis}, we give a visual representation of the two transformations in which the environment and the objects are roto-translated while the robot is fixed (a) and the objects on the table are rotated around the last position of the original trajectory (b). Given a roto-translation of the environment $R$ around a center $c = (x_{c} ,\ y_{c} ,\ z_{c}) $, the transformation is applied to the simulation environment (except the robot) and action sequence $\mathbf{A}$ (as we control the robot by end-effector positions). The generated trajectory is executed on the transformed environment to collect the observations and check that the goal reached by the objects $\hat{g_i}$ is close to the transformed $g_i$. This condition can be expressed as $ ||\hat{g_i} - R_i (g_i - c_i) + c_i || < th $, where $th=0.015$ is an empirical distance in meters.

The second transformation is obtained by rotating the objects and the trajectory with $c_i$ equal to the last position of the set of actions $\mathbf{A}$. $R_i$ can be applied to the all the $a_{pose}$ and the intractable objects, keeping the  demonstration consistent with the task.
As for the previous augmentation, the trajectory and the generated environment are tested to collect the observation and check that the objects reach the final goal position.


%The physics-powered world model is used to create a synthetic set $\mathcal{D}_{aug}$. Given the demonstration $d_i$, the set of actions $\mathcal{A}$ should be equivariant to any rigid transformation of the environment that allows the objects to reach the goal $g_i$. For example, given a rotation of the objects and table $RE_i$ around a center $CE_i = (x_{ci}\,y_{ci}\,z_{ci}) $, we can apply the same rotation to $\mathcal{A}$ to correctly reach $g_i$. However, we also have to consider whether the new trajectory is outside the robot's workspace or if it could contain a singular position. We can directly check that in the world model by playing the trajectory and checking if the goal reached by each object $\hat{g_i}$ is close to the transformed $g_i$. This approach is also used to extract the data since we can render the new observations through the gaussians. 

% The condition could be formalize as:
% \begin{equation}
%    ||\hat{g_i} - RE_i (g_i - CE_i) + CE_i || < th 
%    \label{eq:goal_equation}
%  \end{equation}
% where $th=0.015$ is an empirical distance.


==> text/old_text/experiments-Sep29.tex <==
\section{Experiments}
\label{sec:experiemnts}

In this section, we study the performance of \name with imagination data in comparison with imitation learning agents that have access only to original demonstrations from humans. We test \name using both simulated and real-world environments. For these experiments, PerAct~\citep{shridhar2023perceiveractor} is used as an agent since it is a common baseline for imitation learning. Specifically, we address the following questions:

	1.	How does \name learn when a few demonstrations are available in both single-task and multi-task settings? Is our manipulation world model still useful when more demonstrations are available?
	2.  How do different components of \name affect final performance? 
	3.	How does \name scale to real-world tasks where both imitation and world model learning become more challenging?

\subsection{One-shot Single- and Multi-task Policy Learning}
First, we test how \name performs in the challenging regime with a minimal number of demonstrations in each task, i.e., one example for each task variation~(or $3$-$5$ demonstrations per task). We start by learning a manipulation world model~(\sec{sec:learning_to_imagine}) and then
% ensure that the demonstrations for each task are replayable, i.e., leading to the similar final states are demonstrations final states (see X) \str{This is a bit unclear}. Then, 
we generate new demonstrations by transforming each demonstration's initial state and executing transformed actions~(\sec{sec:imagining_to_learn}). Finally, we train \name on both only imagined demonstrations from the manipulation world model and on a combination of those and original demonstrations.\looseness=-1 
% \str{This paragraph should be written a bit more clearly.}

\label{sec:single_task_results}
\paragraph{Data Collection in Simulation} Following the original implementation of PerAct, we conduct the experiments on RLBench~\citep{james2020rlbench}. The environment is composed of a Franka Emika Panda with a parallel jaw gripper placed on top of a table, and a set of objects, depending on the task, with varying colors and positions. RLBench contains several tasks, we focus on the subset without articulated objects (e.g., drawers), because our object-centric priors do not account for articulations yet. To illustrate how \name performs in different settings, we include two types of tasks: 1. non-prehensile tasks like \textit{slide block}, and 2. pick-and-place tasks like \textit{close jar} and \textit{place shape}. Similar to~\citet{ze2023gnfactor}, the images $\mathcal{I}$ consist of $200$ images collected by simulating a rotating camera around the scene.
While in the real robot scenes the foundational segmentation model~\citep{ren2024grounded} worked well, in the simulated scenes in RLBench, the segmentation model underperformed because most likely it was not trained extensively on synthetic data~(see~\app{app:seg_gap}).
As our primary focus is anyway on real robot data, for the real robot data, we use the foundational segmentation model, and for the synthetic data, we use the ground-truth segmentations of the objects.\looseness=-1
% Since there is a domain gap between the RLBench renderings and natural images that affects the performance of the foundational segmentation model~\citep{ren2024grounded}, we used the ground-truth segmentations of the objects in  (see ~\app{app:seg_gap}).\looseness=-1


% In addition to single-task training, PerAct is designed to handle multi-task setting, where the same model has learned a policy that adapts to more objectives based on the prompt received. 
PerAct is designed to handle multi-task setting in addition to single-task training. In this setting, the same model learns a single policy that adapts to multiple tasks based on the prompts it receives, leading to a more practical and general policy.
We train PerAct and \name models simultaneously on three tasks using the same demonstrations as for single-task training. We use the same hyperparameters for training, except for the number of iterations, which was increased to 600k as in the original paper~\citep{shridhar2023perceiveractor}. To avoid overfitting, in both settings, we validate the performance of each model on a validation set every 10k iterations and select the best-performing model.\looseness=-1 

\paragraph{Single-task and Multi-task Results} 
We report the success rate of the agents trained in both single- and multi-task settings in ~\tab{tab:combined_results}. In addition to the comparison with PerAct~(first raw), we train \name using only imagined demonstrations~(second raw) as well as on the combination of imagined and original demonstrations~(third raw). 
%Results on the multi-task setting, instead, consider also two more agents: C2F-arm~\citep{james2022coarsec2farm}, which is an offline RL approach, and RVT-2~\citep{goyal2024rvt2} that is state of the art in imitation learning. 
As the few demonstrations available are not enough to learn a general policy, the PerAct model trained in the original data performs the worst. By contrast, while using the same original data, \name significantly outperforms PerAct in both single-task and multi-task settings~(+X on single task +Y on multi-task), showing that additional imagination demonstrations help create more robust policies, even when a few demonstrations are available. In multi-task training, the agent trained with imagination and real data together has the highest accuracy, except for the \textit{place shape} task. This may be caused by suboptimal sampling during training since the \textit{close jar} and the \textit{slide block} tasks have more training examples~(see \app{app:learning_details}). 
In addition, we confirm the observation by~\citet{shridhar2023perceiveractor} that with multi-task learning, the agent can complete different tasks, however, at the expense of lower accuracies per task.

Interestingly, \name trained on \emph{only imagination demonstrations} and evaluated in a zero-shot manner afterward still performs significantly better than PerAct (+X on single task +Y on multi-task). This shows that learning behaviors entirely in imagination could be a good strategy if the learned manipulation world model is accurate enough.
% The selected model was tested five times since the agent directly interacts with the simulation, creating some aleatory phenomena (see~\cite{goyal2024rvt2}). 
 % The benefit of the imagination is visible when we exploit this capability to generate data with new configurations, with an average gain of $4.3\%$ on the mean accuracy. 
% We report the success rate of the agents in ~\tab{tab:combined_results}.
% As the few demonstrations available are not enough to learn a general policy, the model trained in the original data performs the worst.
% The accuracy obtained by the multi-task agents is lower to the accuracy obtained by training the agent on single tasks.
% Despite not being intuitive it is similar to what the authors demonstrated in the original paper~\citep{shridhar2023perceiveractor}.
% By contrast, when including imaginations generated by \name, especially when combined with the original training data that is anyway available, we see a significant increase.
% \str{I think the names of the methods should be better clarified. Sim only is still VividDreamer, no?}
% The results demonstrate that imagination data is helping in the multi-task setting, particularly when mixed with real demonstrations.


\begin{table}[tb]
\caption{Comparison of PerAct~\citep{shridhar2023perceiveractor} trained on specific tasks and in a multi-task setting with original data, imagination data, and mixed data. The table reports the average accuracy of five test runs and the maximum accuracy reached.}
\begin{center}
\resizebox{\columnwidth}{!}{
 \begin{tabular}{@{}lcccccc cc @{}}\toprule
 \multirow{3}{*}{} & \multicolumn{8}{c}{\textbf{Single-task}} \\
 \cmidrule(lr){2-9} %\cmidrule(lr){8-15} 
& \multicolumn{2}{c}{\textit{close jar}} & \multicolumn{2}{c}{\textit{place shape}} & \multicolumn{2}{c}{\textit{slide block}} & \multicolumn{2}{c}{\textit{avg single-task}}  \\
& Mean $\pm$ Std & Max & Mean $\pm$ Std & Max & Mean $\pm$ Std & Max & Mean & Max \\
 \midrule
 PerAct & 38.4 $\pm$ 0.64 & 40 & 6.4 $\pm$ 2.24 & 8 & 48.4 $\pm$ 10.24 & 50 & & \\
 \name~\textit{(Sim. only)} & 41.2 $\pm$ 5.76 & 46 & 9.6 $\pm$ 2.24 & 12 & 54.4 $\pm$ 4.64 & 62 & & \\
 \name~\textit{(All data)} & \textbf{51.2} $\pm$ 2.56 & \textbf{54} & \textbf{11.2} $\pm$ 2.56 & \textbf{12} & \textbf{62.0} $\pm$ 4.80 & \textbf{66} & & \\

\midrule
\multirow{3}{*}{} & \multicolumn{8}{c}{\textbf{Multi-task}} \\
\cmidrule(lr){2-9}
\multirow{3}{*}{} & \multicolumn{2}{c}{\textit{close jar}} & \multicolumn{2}{c}{\textit{place shape}} & \multicolumn{2}{c}{\textit{slide block}} & \multicolumn{2}{c}{\textit{avg multi-task}} \\

& Mean $\pm$ Std & Max & Mean $\pm$ Std & Max & Mean $\pm$ Std & Max & Mean & Max \\
\midrule
PerAct & 26.0 $\pm$ 9.60 & 28 & 7.2 $\pm$ 2.56 & 10 & 34.0 $\pm$ 25.60 & 38 & 22.4 & 25.3 \\
\name~\textit{(Sim. only)} & 28.0 $\pm$ 11.20 & 32 & \textbf{18.0} $\pm$ 8.0 & \textbf{22} & 48.0 $\pm$ 3.20 & 50 & 31.3 & 34.7\\
\name~\textit{(All data)} & \textbf{46.0} $\pm$ 12.8 & \textbf{52} & 6.4 $\pm$ 10.24 & 12 & \textbf{54.0} $\pm$ 4.80 & \textbf{58} & \textbf{35.5} & \textbf{40.7}  \\
\bottomrule
\end{tabular}
}
\end{center}
\label{tab:combined_results}
\end{table}


% \begin{table}[tb]
% \caption{Results of PerAct~\citep{shridhar2023perceiveractor} trained on a specific task with original data, imagination data, and mixed data. The table reports the average accuracy of five test runs and the maximum accuracy reached.}
% \begin{center}
% \resizebox{0.8\columnwidth}{!}{
% \begin{tabular}{@{}l|cc|cc|cc@{}}\toprule
        
%         \multirow{2}{*}{Name} & \multicolumn{2}{c|}{\textit{close jar}} & \multicolumn{2}{c|}{\textit{place shape}} & \multicolumn{2}{c}{\textit{slide block}}\\
%                               &  Mean $\pm$ Std        & Max& Mean $\pm$ Std         & Max& Mean $\pm$ Std          & Max \\    \midrule
%         PerAct    & 38.4 $\pm$ 0.64 & 40 & 6.4 $\pm$ 2.24  &  8 & 48.4 $\pm$ 10.24 & 50  \\
%         % \midrule
%         \name~\textit{(Sim. only)} & 41.2 $\pm$ 5.76 & 46 & 9.6  $\pm$ 2.24 & 12 & 54.4 $\pm$  4.64 & 62  \\
%         \name          & \textbf{51.2} $\pm$ 2.56  & \textbf{54} & \textbf{11.2} $\pm$ 2.56 & \textbf{12} & \textbf{62.0} $\pm$  4.80 & \textbf{66}  \\
%         \bottomrule
      
%     %\bottomrule
% \end{tabular}
% }
% \end{center}
% \label{tab:results_single_task}
% \end{table}

% \begin{table}[t]
% \caption{Results of PerAct~\citep{shridhar2023perceiveractor} trained in a multi-task setting with original data, imagination data, and mixed data. The table reports the average accuracy of five test iterations and the maximum accuracy reached.}
% \begin{center}
% \resizebox{0.9\columnwidth}{!}{
% \begin{tabular}{@{}l|cc|cc|cc|cc@{}}\toprule
%     \multirow{2}{*}{Name} & \multicolumn{2}{c|}{\textit{close jar}} & \multicolumn{2}{c|}{\textit{place shape}} & \multicolumn{2}{c|}{\textit{slide block}} & \multicolumn{2}{c}{\textit{average multi-task}}\\
%                          & Mean $\pm$ Std & Max & Mean $\pm$ Std & Max & Mean $\pm$ Std & Max & Mean & Max \\    \midrule
%     PerAct                & 26.0 $\pm$ 9.60 & 28 & 7.2 $\pm$ 2.56 & 10 & 34.0 $\pm$ 25.60 & 38 & 22.4 & 25.3 \\
%     % \midrule
%     % Trajectory          &        &       &        &      &        &     &        &      \\
%     % Roto-translation    & 28.0 $\pm$ 11.20 & 32 & \textbf{18.8} $\pm$ 36.16 & \textbf{26} & 44.0 $\pm$ 1.60 & 46 & 30.3 & 34.7 \\
%     \name~\textit{(Sim. only)}                 & 28.0 $\pm$ 11.20 & 32 & 18.0 $\pm$ 8.0 & 22 & 48.0 $\pm$ 3.20 & 50 & 31.3 & 34.7 \\
%     % \midrule
%     \name         & \textbf{46.0} $\pm$ 12.8 & \textbf{52} & 6.4 $\pm$ 10.24 & 12 & \textbf{54.0} $\pm$ 4.80 & \textbf{58} & \textbf{35.5} & \textbf{40.7} \\
% \bottomrule
% \end{tabular}
% }
% \end{center}

% \label{tab:results_multi_task}
% \end{table}

\subsection{Analysis and ablation study}

\paragraph{Varying dataset size}

\begin{table}[tb]
\caption{Performance of \name train on single-task demonstrations from different types of transformations. The table reports the average accuracy of five test runs and the maximum accuracy reached.}
\begin{center}
\resizebox{0.8\columnwidth}{!}{
\begin{tabular}{@{}l|cc|cc|cc@{}}\toprule
        
        \multirow{2}{*}{Name} & \multicolumn{2}{c|}{\textit{close jar}} & \multicolumn{2}{c|}{\textit{place shape}} & \multicolumn{2}{c}{\textit{slide block}}\\
                              &  Mean $\pm$ Std        & Max& Mean $\pm$ Std         & Max& Mean $\pm$ Std          & Max \\    \midrule
        % Real                  & 38.4 $\pm$ 0.64 & 40 & 6.4 $\pm$ 2.24  &  8 & 48.4 $\pm$ 10.24 & 50  \\
        % \midrule
        Replay                & 10.0 $\pm$ 9.60 & 16 & 1.2 $\pm$ 0.96  &  2 & 26.0 $\pm$ 0.00  & 26  \\ 

        Object Rotation      & 25.2 $\pm$ 0.96 & 26 & 10.4 $\pm$ 7.04 & \textbf{14} & 42.0 $\pm$  0.00 & 42  \\
        %Trajectory + Real     & 5 + 52  & 22.4 $\pm$ 2.24 & 24 & 5 + 31 & $\pm$           &    & 4 + 15 & 51.6 $\pm$  0.64 & 52  \\
        Roto-translation      & 41.2 $\pm$ 5.76 & 44 & 10.0 $\pm$ 6.40 & \textbf{14} & 50.4 $\pm$  2.24 & 52  \\
        %Augmented + Real      & 5 + 65  & 34.0 $\pm$ 8.00 & 38 & 5 + 55 & 10.0 $\pm$ 8.00 & 14 & 4 + 50 & 53.2 $\pm$  2.56 & 56  \\

        \name           & \textbf{51.2} $\pm$ 2.56  & \textbf{54} & \textbf{11.2} $\pm$ 2.56 & 12 & \textbf{62.0} $\pm$  4.80 & \textbf{66}  \\
        \bottomrule
      
    %\bottomrule
\end{tabular}
}
\end{center}
\label{tab:results_single_task}
\end{table}



% \subsection{Varying dataset size}
\label{sec:increasing_data} We analyze how effective \name's imagined augmentations are depending on the number of original demonstrations provided. 
% verify the agent's behaviour when trained incrementing the real data and the imagination data. 
For this, we vary dataset size $|\mathcal{D}| \in \{4, 10, 20\}$ for the \textit{slide block} and \textit{place shape} tasks since they are the best and worst in the previous experiment. The generated imagination data with rotation of the trajectory and roto-translation of the environment for the \textit{slide block} from the $10$ and $20$ examples is $167$ and $391$ examples respectively, and the generated data for the \textit{place shape} is $176$ and $437$ examples. 

We trained the models as in the previous experiment: 100k with batch 4 and the original parameters for the optimizer. We tested the best validation model five times and reported the average and the maximum accuracy in solving the task. \Fig{fig:increasing_data_results} reports the average accuracy of PerAct with new sets of demonstrations. Increasing the training examples to 20 improves the results in both tasks. The original data have better quality since the agent trained with 20 examples can match or pass the accuracy of the one trained with imagination data from 5 examples (81 examples for \textit{place shape} and 61 examples for the \textit{slide block}). However, thanks to the ability to imagine and increasing the data distribution, when the 20 examples are used to generate the imagination data the model gains $6.4\%$ and $10.4\%$ respectively. ~\Fig{fig:distribution} shows that incrementing the original data with imagination data allows it to cover a wider area of the space. With 20 examples, the keypoints from the imagination data cover a wider portion of the workspace empowering the agent to understand how to behave in configurations far from the original ones. 

\paragraph{Transformation Ablation Study} To better understand the effectiveness of proposed equivariant transformations, we perform an additional ablation study, ablating which transformations are used for augmentation.  We create 6 splits of data: \textit{Real}, \textit{Replay}, \textit{Trajectory}, \textit{Roto-translation}, \textit{All} and \textit{All + Real}. The \textit{Real} split contains only real data $\mathcal{D}$, whereas the \textit{Replay} split contains imagination data generated using the demonstrated trajectories. \textit{Trajectory} and \textit{Roto-translation} augmentations contain data generated using the two proposed equivariant transformations. Finally, the \textit{All} split contains both the data and the \textit{All + Real} contains both the imagination data and the real data.
% For each split, PerAct was trained for 100k iterations on an Nvidia A40 with 48GB and a batch size of 4 saving a model every 5k iterations.
% Similarly to the authors of the PerAct, we extracted $40$ scenarios as validation to select which model to test and $50$ examples as a test set. 

% \paragraph{Results} 

As we explain in the following experiment (\sec{sec:increasing_data}), the equivariant transformations used for the \textit{Trajectory} and \textit{Roto-translation} splits allow to expand the training distribution and improve the generalization of the learned policy. The best results are understandably obtained by mixing the imagination with the real data with an average improvement of 10.4\% on the mean accuracy. 

\begin{figure}[t]
\centering
\includegraphics[width=0.4\textwidth]{ICLR 2025 Template/images/incrementing_slide_block_average.png}
\includegraphics[width=0.4\textwidth]{ICLR 2025 Template/images/incrementing_place_shape_average.png} 
\\
\caption{Results increasing the training examples for the \textit{slide block} task (left) and  \textit{place shape} task (right). In blue the results with the real data, while in red the with imagination created using the same number real examples.}
\label{fig:increasing_data_results}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=0.325\textwidth]{images/place_shape_incremented_1example_keypoints_v2.png}
\includegraphics[width=0.325\textwidth]{images/place_shape_incremented_5example_keypoints_v2.png} 
\includegraphics[width=0.325\textwidth]{images/place_shape_incremented_20example_keypoints_v2.png} 
\\
\caption{Keypoints distribution of original (blue dots) and generated data (red cross) for the \textit{place shape} task. Data is generated from one examples (left), five examples (middle) and twenty examples (right). }
\label{fig:distribution}
\end{figure}




\subsection{Results of Real Robot Experiments}
\label{sec:real_experiment}

\paragraph{Robot Setup} We verified that our approach works also in real environments. Our setup comprises a Franka Emika Panda on a table with a calibrated Kinect Azure mounted on the end-effector. A Kinect V2 is positioned in front of the table mimicking the real experiment done in PerAct. We collected examples for three tasks: a pick and place of a block (named \textit{pick block}), a pick and place of different shapes (\textit{pick shape}) and a push task (\textit{push}). The first has two variations in the place position, the second task has three variations in the pick, and the last has only one variation. We collected respectively 4, 5 and 3 demonstrations. For each demonstration, we collected images of the environment and we applied our method to create the world model and sample new data using the equivariant transformations. We trained two models for each task, one using only original data and the other with imagination and real data, with the same hyper-parameters of ~\sec{sec:single_task_results}. More information about the tasks and the generation are available in the Appendix.

\paragraph{Test Results with Mixed Imagination} We checked the last five models produced in training five configurations of objects similar to the training and selected the best performing model. We tested the selected model in 20 configurations of the environment: 10 with positions of objects similar to the original training data and 10 with position out of the distribution to test whether the models generalize to configurations not in the real training set. The results are reported in ~\Tab{tab:results_real}, confirming that the data generated in is helping the model to perform the tasks. In particular, the models trained on real data encountered problems in the distribution of the objects different form the originals. The place shape is the task with lower accuracy. This is caused by the small size of the shape and the difficulty that the model had in recognize the correct one. We noticed that the depth of kinect v2 is not good enough to correctly represent the different shapes probably impacting in the task.

\paragraph{Test Results with Pure Imagination} We checked the last five models produced in training five configurations of objects similar to the training and selected the best performing model. We tested the chosen model in 20 configurations of the environment: 10 with positions of objects close to the one used in the training demonstrations and 10 with positions out of the distribution to test whether the models generalize to configurations, not in the real training set. The results are reported in ~\Tab{tab:results_real}, confirming that the data generated is helping the model to perform the tasks. In particular, the models trained on real data encountered problems in the distribution of the objects different from the originals. The place shape is the task with lower accuracy. This is caused by the small size of the shape and the difficulty that the model had in recognising the correct one. We noticed that the depth of Kinect v2 is not good enough to correctly represent the different shapes, probably impacting the agent accuracy.

% GENERATED DATA -> slide block 169, push block 31, place shape 85, pick block 183 (8 examples) and 94 (4 examples)

% \begin{table}[h]
% \caption{}
% \begin{center}
% \resizebox{0.6\columnwidth}{!}{
% \begin{tabular}{@{}l|cc|cc@{}}\toprule
%         \multirow{2}{*}{Name} & \multicolumn{2}{c|}{Results}  & \multicolumn{2}{c}{Out of distribution results}   \\
%                             & 8 examples     &    4 examples  & 8 examples             &    4 examples      \\ 
%         \midrule
%         Real                & 65 & 55 & 50 & 50 \\
%         \midrule
%         All                 & \textbf{85} & 50 & \textbf{80} & 20 \\
%         \midrule
%         All + Real          & \textbf{85} & \textbf{90} & 70 & \textbf{80} \\
%     \bottomrule
% \end{tabular}
% }
% \end{center}

% \label{tab:results_real_pick_place_block}
% \end{table}

\begin{table}[h]
\caption{Results of the real experiment with original and original mixed with imagination data.}
\begin{center}
\resizebox{0.8\columnwidth}{!}{
\begin{tabular}{@{}l|cc|cc|cc@{}}\toprule
            
        \multirow{2}{*}{Name}& \multicolumn{2}{c|}{pick  block (4 examples)} & \multicolumn{2}{c|}{pick shape} & \multicolumn{2}{c}{push}  \\
        & Results & Results OOD  & Results & Results OOD  & Results & Results OOD \\
        \midrule
        Real                 & 55 & 50 & 30 & 10 & 40 & 10 \\
        \midrule
        Imagination + Real   & \textbf{90} & \textbf{90} & \textbf{35} & \textbf{30} & \textbf{80} & \textbf{60} \\
    \bottomrule
\end{tabular}
}
\end{center}

\label{tab:results_real}
\end{table}


\begin{table}[h]
\caption{Results of the \textit{Pick Block} task with original and imagination data.}
\begin{center}
\resizebox{0.5\columnwidth}{!}{
\begin{tabular}{@{}l|c|c@{}}\toprule
            
        \multirow{1}{*}{Name}& \multicolumn{1}{c|}{Results 4 examples} & \multicolumn{1}{c}{Results 8 examples}  \\
        \midrule
        Real                 & \textbf{55} & 55 \\
        \midrule
        Imagination           & 50 & \textbf{80} \\
    \bottomrule
\end{tabular}
}
\end{center}

\label{tab:results_real_pick_place_block}
\end{table}

==> text/old_text/experiments_old.tex <==
\section{Experiments}
\label{sec:experiemnts}

In this section, we present the results of the imitation learning agents trained using imagination data obtained from our manipulation world model. The equivariant generation is tested in simulation and a real scenario. First, the single-task results with limited examples are presented. Then, we study the agent's behaviour when 10 and 20 examples are available. For these experiments, PerAct~\citep{shridhar2023perceiveractor} is used as an agent since it is a common baseline for imitation learning. Then, the same model is tested in a multi-task setting to verify that the world model can also help generalize in this configuration. Finally, the entire framework is tested in a real scenario to prove that we can automatically reconstruct the world model in real scenarios and deploy it to collect imagination demonstrations that improve the generalizability of the agent.

%Results on multi-task setting, instead, considers also two more agents: C2F-arm~\citep{james2022coarsec2farm}, that is a offline RL approach, and RVT-2~\citep{goyal2024rvt2} that is state of the art in imitation learning. 

\subsection{Single-task results}
\label{sec:single_task_results}
\paragraph{Data Collection in Simulation} Following the original implementation of PerAct, we conducted the experiments on RLBench~\citep{james2020rlbench}. The environment is composed of a Franka Emika Panda with a parallel jaw gripper placed on top of a table, and a set of objects, depending on the task, with varying colors and positions. RLBench comprehends several tasks, but we selected only a subset without articulated objects (e.g. drawers). We included two types of tasks: non-prehensile tasks, i.e. \textit{slide the block}, and pick-and-place tasks, i.e. \textit{close jar} and \textit{place shape in shape sorter}.
For the pick and place tasks, we collected $\mathcal{D}$ with a cardinality of 5 while for the slide task with a cardinality of 4, i.e.~one example for each variation. The set $\mathcal{I}$ was collected by simulating a camera and making it rotate around the scene similarly to~\citet{ze2023gnfactor} to collect 200 images. Since the data are synthetic and there is a domain gap between the real images and the RLBench renderings, we used the ground-truth segmentation of the objects to generate the world models (see ~\app{app:seg_gap}).

\paragraph{Training and Testing} We created 6 splits of data: \textit{Real}, \textit{Replay}, \textit{Trajectory}, \textit{Roto-translation}, \textit{All} and \textit{All + Real}. The \textit{Real} split contains only real data $\mathcal{D}$, whereas the \textit{Replay} split contains imagination data generated using the demonstrated trajectories. \textit{Trajectory} and \textit{Roto-translation} augmentations contain data generated using the two proposed equivariant transformations. Finally, the \textit{All} split contains both the data and the \textit{All + Real} contains both the imagination data and the real data.
For each split, PerAct was trained for 100k iterations on an Nvidia A40 with 48GB and a batch size of 4 saving a model every 5k iterations.
Similarly to the authors of the PerAct, we extracted 40 scenarios as validation to selecte which model to test and 50 examples as test set. 

\paragraph{Results} The selected model was tested five times since the agent directly interacts with the simulation, creating some aleatory phenomena (see~\cite{goyal2024rvt2}). The results reported in~\Tab{tab:results_single_task} demonstrate that imagination data helps create general policies when few demonstrations are available. The real data has a higher quality since the \textit{Replay} has lower accuracy. The benefit of the imagination is visible when we exploit this capability to generate data with new configurations, with an average gain of 4.3\% on the mean accuracy. As we explain in the following experiment (\sec{sec:increasing_data}), the equivariant transformations used for the \textit{Trajectory} and \textit{Roto-translation} splits allow to expand the training distribution and improve the generalization of the learned policy. The best results are understandably obtained by mixing the imagination with the real data with an average improvement of 10.4\% on the mean accuracy. 


% \begin{table}[h]
% \caption{Single task results}
% \begin{center}
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{@{}l|ccc|ccc|ccc@{}}\toprule
        
%         \multirow{2}{*}{Name} & \multicolumn{3}{c|}{Close jar} & \multicolumn{3}{c|}{Place Shape} & \multicolumn{3}{c}{Slide block}\\
%                               & Examples& Results         & Max&Examples& Results         & Max&Examples& Results          & Max \\    \midrule
%         Real                  & 5 + 0   & 37.2 $\pm$ 5.76 & 40 & 5 + 0  & 6.4 $\pm$ 2.24  &  8 & 4 + 0  & 48.4 $\pm$ 10.24 & 50  \\
%         \midrule
%         Replay                & 0 + 5   & $\pm$           &    & 0 + 5  & $\pm$           &    & 0 + 4  & $\pm$            &   \\
%         Trajectory            & 0 + 52  & 24.0 $\pm$ 4.80 & 26 & 0 + 31 & 10.4 $\pm$ 7.04 & 14 & 0 + 15 & 42.0 $\pm$  0.00 & 42  \\
%         %Trajectory + Real     & 5 + 52  & 22.4 $\pm$ 2.24 & 24 & 5 + 31 & $\pm$           &    & 4 + 15 & 51.6 $\pm$  0.64 & 52  \\
%         Roto-translation      & 0 + 65  & 36.8 $\pm$ 7.34 & 40 & 0 + 55 & 10.0 $\pm$ 6.40 & 14 & 0 + 50 & 50.4 $\pm$  2.24 & 52  \\
%         %Augmented + Real      & 5 + 65  & 34.0 $\pm$ 8.00 & 38 & 5 + 55 & 10.0 $\pm$ 8.00 & 14 & 4 + 50 & 53.2 $\pm$  2.56 & 56  \\
%         All                   & 0 + 112 & 44.0 $\pm$ 3.20 & 46 & 0 + 81 & $\pm$           &    & 0 + 61 & 54.4 $\pm$  4.64 & 62  \\
%         %All + Real            & 5 + 112 & 27.6 $\pm$ 2.24 & 30 & 5 + 81 & $\pm$           &    & 4 + 61 & 62.0 $\pm$  4.80 & 66  \\
%         %\midrule
%         %Best augmentation     & 0 + 112 & 44.0 $\pm$ 3.20 & 46 & 0 + 31 & 10.4 $\pm$ 7.04 & 14 & 4 + 61 & 62.0 $\pm$  4.80 & 66 \\
%         \bottomrule
      
%     %\bottomrule
% \end{tabular}
% }
% \end{center}
% \label{tab:results_ntu}
% \end{table}

\begin{table}[tb]
\caption{Results of PerAct~\citep{shridhar2023perceiveractor} trained on a specific task with original data, imagination data, and mixed data. The table reports the average accuracy of five test runs and the maximum accuracy reached.}
\begin{center}
\resizebox{0.8\columnwidth}{!}{
\begin{tabular}{@{}l|cc|cc|cc@{}}\toprule
        
        \multirow{2}{*}{Name} & \multicolumn{2}{c|}{\textit{close jar}} & \multicolumn{2}{c|}{\textit{place shape}} & \multicolumn{2}{c}{\textit{slide block}}\\
                              &  Mean $\pm$ Std        & Max& Mean $\pm$ Std         & Max& Mean $\pm$ Std          & Max \\    \midrule
        Real                  & 38.4 $\pm$ 0.64 & 40 & 6.4 $\pm$ 2.24  &  8 & 48.4 $\pm$ 10.24 & 50  \\
        \midrule
        Replay                & 10.0 $\pm$ 9.60 & 16 & 1.2 $\pm$ 0.96  &  2 & 26.0 $\pm$ 0.00  & 26  \\ 
        \midrule
        Trajectory            & 25.2 $\pm$ 0.96 & 26 & 10.4 $\pm$ 7.04 & 14 & 42.0 $\pm$  0.00 & 42  \\
        %Trajectory + Real     & 5 + 52  & 22.4 $\pm$ 2.24 & 24 & 5 + 31 & $\pm$           &    & 4 + 15 & 51.6 $\pm$  0.64 & 52  \\
        Roto-translation      & 41.2 $\pm$ 5.76 & 44 & 10.0 $\pm$ 6.40 & 14 & 50.4 $\pm$  2.24 & 52  \\
        %Augmented + Real      & 5 + 65  & 34.0 $\pm$ 8.00 & 38 & 5 + 55 & 10.0 $\pm$ 8.00 & 14 & 4 + 50 & 53.2 $\pm$  2.56 & 56  \\
        All                   & 41.2 $\pm$ 5.76 & 46 & 9.6  $\pm$ 2.24 & 12 & 54.4 $\pm$  4.64 & 62  \\
        %All + Real            & 5 + 112 & 27.6 $\pm$ 2.24 & 30 & 5 + 81 & $\pm$           &    & 4 + 61 & 62.0 $\pm$  4.80 & 66  \\
        %\midrule
        %Best augmentation     & 0 + 112 & 44.0 $\pm$ 3.20 & 46 & 0 + 31 & 10.4 $\pm$ 7.04 & 14 & 4 + 61 & 62.0 $\pm$  4.80 & 66 \\
        \midrule
        All + Real            & \textbf{51.2} $\pm$ 2.56  & \textbf{54} & \textbf{11.2} $\pm$ 2.56 & \textbf{12} & \textbf{62.0} $\pm$  4.80 & \textbf{66}  \\
        \bottomrule
      
    %\bottomrule
\end{tabular}
}
\end{center}
\label{tab:results_single_task}
\end{table}

\subsection{Varying dataset size}
\label{sec:increasing_data}
\paragraph{Data Collection} We analyze how effective \name's imagined augmentations are depending on the number of original demonstrations provided. 
% verify the agent's behaviour when trained incrementing the real data and the imagination data. 
For this, we vary dataset size $|\mathcal{D}| \in \{4, 10, 20\}$ for the \textit{slide block} and \textit{place shape in shape sorter} tasks since they are the best and worst in the previous experiment. The generated imagination data with rotation of the trajectory and roto-translation of the environment for the \textit{slide block} from the $10$ and $20$ examples is $167$ and $391$ examples respectively, and the generated data for the \textit{place shape in shape sorter} is $176$ and $437$ examples. 

\paragraph{Results} We trained the models as in the previous experiment: 100k with batch 4 and the original parameters for the optimizer. We tested the best validation model five times and reported the average and the maximum accuracy in solving the task. \Fig{fig:increasing_data_results} reports the average accuracy of PerAct with new sets of demonstrations. Increasing the training examples to 20 improves the results in both tasks. The original data have better quality since the agent trained with 20 examples can match or pass the accuracy of the one trained with imagination data from 5 examples (81 examples for \textit{place shape in shape sorter} and 61 examples for the \textit{slide block}). However, thanks to the ability to imagine and increasing the data distribution, when the 20 examples are used to generate the imagination data the model gains $6.4\%$ and $10.4\%$ respectively. ~\Fig{fig:distribution} shows that incrementing the original data with imagination data allows it to cover a wider area of the space. With 20 examples, the keypoints from the imagination data cover a wider portion of the workspace empowering the agent to understand how to behave in configurations far from the original ones. 

\begin{figure}[t]
\centering
\includegraphics[width=0.4\textwidth]{ICLR 2025 Template/images/incrementing_slide_block_average.png}
\includegraphics[width=0.4\textwidth]{ICLR 2025 Template/images/incrementing_place_shape_average.png} 
\\
\caption{Results increasing the training examples for the \textit{slide block} task (left) and  \textit{place shape in shape sorter} task (right). In blue the results with the real data, while in red the with imagination created using the same number real examples.}
\label{fig:increasing_data_results}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=0.325\textwidth]{images/place_shape_incremented_1example_keypoints_v2.png}
\includegraphics[width=0.325\textwidth]{images/place_shape_incremented_5example_keypoints_v2.png} 
\includegraphics[width=0.325\textwidth]{images/place_shape_incremented_20example_keypoints_v2.png} 
\\
\caption{Keypoints distribution of original (blue dots) and generated data (red cross) for the \textit{place shape in shape sorter} task. Data is generated from one examples (left), five examples (middle) and twenty examples (right). }
\label{fig:distribution}
\end{figure}

\subsection{Multi-task results}

Peract is designed to work in multi-task settings where the same model has learnt a policy that adapts to more objectives based on the prompt received. Therefore, we trained the model with the same splits of~\sec{sec:single_task_results} but simultaneously on the three tasks. We trained a model for each split, keeping the same parameter except for the number of iterations, which was increased to 600k as in the original paper. One model every 10k iterations is saved and the best model is selected using the validation. 

\paragraph{Results} The accuracy of the agents are reported in ~\Tab{tab:results_multi_task}. The model trained in the original data is the worst-performing one since the few demonstrations available are not enough to learn a general policy. The accuracy obtained by the multi-task agents is lower to the accuracy obtained by training the agent on single tasks. Despite not being intuitive it is similar to what the authors demonstrated in the original paper~\citep{shridhar2023perceiveractor}. The results demonstrate that imagination data is helping in the multi-task setting, particularly when mixed with real demonstrations. The agent trained with imagination and real data together has the highest accuracy except for the \textit{place shape in shape sorter} task. This may be caused by sub-optimal sampling during training since the "close jar" and the "slide block" tasks have more training examples. 

\begin{table}[t]
\caption{Results of PerAct~\citep{shridhar2023perceiveractor} trained in a multi-task setting with original data, imagination data and mixed data. The table reports the average accuracy of five test iteration and the maximum accuracy reached.}
\begin{center}
\resizebox{0.9\columnwidth}{!}{
\begin{tabular}{@{}l|cc|cc|cc|cc@{}}\toprule
        \multirow{2}{*}{Name} & \multicolumn{2}{c|}{Average} & \multicolumn{2}{c|}{Close jar} & \multicolumn{2}{c|}{Slide block} & \multicolumn{2}{c}{Place Shape}\\
                            & Mean $\pm$ Std & Max   & Mean $\pm$ Std        & Max& Mean $\pm$ Std         & Max& Mean $\pm$ Std            & Max  \\    \midrule
        Real                &  22.4  & 25.3  & 26.0 $\pm$ 9.60  & 28 & 34.0 $\pm$ 25.60 & 38 & 7.2 $\pm$ 2.56  & 10 \\
        \midrule
        Trajectory          &        &       &     $\pm$         &      &     $\pm$          &     &    $\pm$           &      \\
        %Trajectory + Real  &        &       &     $\pm$         &      &     $\pm$          &     &    $\pm$           &      \\
        Roto-translation    &  30.3  &  34.7 & 28.0 $\pm$ 11.20 & 32 & 44.0 $\pm$ 1.60  & 46 & \textbf{18.8} $\pm$ 36.16 & \textbf{26 }\\
        %Roto-translation   &        &       &     $\pm$         &      &     $\pm$          &     &    $\pm$           &      \\
        All                 &  31.3  &  34.7 & 28.0 $\pm$ 11.20 & 32 & 48.0 $\pm$ 3.20 &  50 & 18.0 $\pm$ 8.0   & 22  \\
        \midrule
        All + Real          &  \textbf{35.5}  &  \textbf{40.7} & \textbf{46.0} $\pm$  12.8 &  \textbf{52 }&  \textbf{54.0} $\pm$  4.80 &\textbf{ 58} & 6.4 $\pm$ 10.24 & 12    \\
    \bottomrule
\end{tabular}
}
\end{center}

\label{tab:results_multi_task}
\end{table}

\subsection{Results of Real Robot Experiments}
\label{sec:real_experiment}

\paragraph{Robot Setup} We verified that our approach works also in real environments. Our setup comprises a Franka Emika Panda on a table with a calibrated Kinect Azure mounted on the end-effector. A Kinect V2 is positioned in front of the table mimicking the real experiment done in PerAct. We collected examples for three tasks: a pick and place of a block (named \textit{pick block}), a pick and place of different shapes (\textit{pick shape}) and a push task (\textit{push}). The first has two variations in the place position, the second task has three variations in the pick, and the last has only one variation. We collected respectively 4, 5 and 3 demonstrations. For each demonstration, we collected images of the environment and we applied our method to create the world model and sample new data using the equivariant transformations. We trained two models for each task, one using only original data and the other with imagination and real data, with the same hyper-parameters of ~\sec{sec:single_task_results}. More information about the tasks and the generation are available in the Appendix.

\paragraph{Test Results with Mixed Imagination} We checked the last five models produced in training five configurations of objects similar to the training and selected the best performing model. We tested the selected model in 20 configurations of the environment: 10 with positions of objects similar to the original training data and 10 with position out of the distribution to test whether the models generalize to configurations not in the real training set. The results are reported in ~\Tab{tab:results_real}, confirming that the data generated in is helping the model to perform the tasks. In particular, the models trained on real data encountered problems in the distribution of the objects different form the originals. The place shape is the task with lower accuracy. This is caused by the small size of the shape and the difficulty that the model had in recognize the correct one. We noticed that the depth of kinect v2 is not good enough to correctly represent the different shapes probably impacting in the task.

\paragraph{Test Results with Pure Imagination} We checked the last five models produced in training five configurations of objects similar to the training and selected the best performing model. We tested the chosen model in 20 configurations of the environment: 10 with positions of objects close to the one used in the training demonstrations and 10 with positions out of the distribution to test whether the models generalize to configurations, not in the real training set. The results are reported in ~\Tab{tab:results_real}, confirming that the data generated is helping the model to perform the tasks. In particular, the models trained on real data encountered problems in the distribution of the objects different from the originals. The place shape is the task with lower accuracy. This is caused by the small size of the shape and the difficulty that the model had in recognising the correct one. We noticed that the depth of Kinect v2 is not good enough to correctly represent the different shapes, probably impacting the agent accuracy.

% GENERATED DATA -> slide block 169, push block 31, place shape 85, pick block 183 (8 examples) and 94 (4 examples)

% \begin{table}[h]
% \caption{}
% \begin{center}
% \resizebox{0.6\columnwidth}{!}{
% \begin{tabular}{@{}l|cc|cc@{}}\toprule
%         \multirow{2}{*}{Name} & \multicolumn{2}{c|}{Results}  & \multicolumn{2}{c}{Out of distribution results}   \\
%                             & 8 examples     &    4 examples  & 8 examples             &    4 examples      \\ 
%         \midrule
%         Real                & 65 & 55 & 50 & 50 \\
%         \midrule
%         All                 & \textbf{85} & 50 & \textbf{80} & 20 \\
%         \midrule
%         All + Real          & \textbf{85} & \textbf{90} & 70 & \textbf{80} \\
%     \bottomrule
% \end{tabular}
% }
% \end{center}

% \label{tab:results_real_pick_place_block}
% \end{table}

\begin{table}[h]
\caption{Results of the real experiment with original and original mixed with imagination data.}
\begin{center}
\resizebox{0.8\columnwidth}{!}{
\begin{tabular}{@{}l|cc|cc|cc@{}}\toprule
            
        \multirow{2}{*}{Name}& \multicolumn{2}{c|}{pick  block (4 examples)} & \multicolumn{2}{c|}{pick shape} & \multicolumn{2}{c}{push}  \\
        & Results & Results OOD  & Results & Results OOD  & Results & Results OOD \\
        \midrule
        Real                 & 55 & 50 & 30 & 10 & 40 & 10 \\
        \midrule
        Imagination + Real   & \textbf{90} & \textbf{90} & \textbf{35} & \textbf{30} & \textbf{80} & \textbf{60} \\
    \bottomrule
\end{tabular}
}
\end{center}

\label{tab:results_real}
\end{table}


\begin{table}[h]
\caption{Results of the \textit{Pick Block} task with original and imagination data.}
\begin{center}
\resizebox{0.5\columnwidth}{!}{
\begin{tabular}{@{}l|c|c@{}}\toprule
            
        \multirow{1}{*}{Name}& \multicolumn{1}{c|}{Results 4 examples} & \multicolumn{1}{c}{Results 8 examples}  \\
        \midrule
        Real                 & \textbf{55} & 55 \\
        \midrule
        Imagination           & 50 & \textbf{80} \\
    \bottomrule
\end{tabular}
}
\end{center}

\label{tab:results_real_pick_place_block}
\end{table}

==> text/old_text/introduction-Sep28.tex <==
\section{Introduction}
\label{sec:Introduction}

% What is a world model and why it important
In robotics, world models are learnable representations of the real world that an agent can use to predict the consequences of its actions~\citep{ha2018worldmodel}. World models give agents the ability to observe the outcomes of actions in imagination, which is crucial for learning new skills~\citep{hafner2019dream, gumbsch2024learning, hansen2024tdmpc} or new behaviours~\citep{pitis2020counterfactual, yang2023learningUnisim}. Thus, they are a fundamental building block for robots to imagine, a capability that we humans exploit to interact with new environments and to learn new skills~\citep{Hawkins2017worldmodel, ha2018worldmodel}.\looseness=-1 

% Explain what it is needed for a grounded world model
Applying world models to real robots implies grounding the representation to the real scenarios in which they need to interact~\citep{yang2023learningUnisim, zhou2024robodreamer} while reliably simulating the dynamics~\citep{li2024evaluating}.
Whereas the world model should behave realistically, the most important characteristic is its usefulness in increasing the knowledge of the robot~\citep{qureshi2024splatsim}. An agent should be capable of interacting with the model and adapting it to explore configurations out of its domain. Moreover, it should connect the real actions of the robot with actions in the world model to bridge what can be learned in imagination into reality~\citep{abou2024physically, torne2024reconciling}.\looseness=-1 

% Current limitations of the apporaches 
One way to create such a world model is by learning a representation by interacting with the environment~\citep{yang2023learningUnisim, zhou2024robodreamer}. Whereas these models generalize to different objectives, predicting the causal consequences of actions falling outside their training distribution can produce hallucinations and unrealistic interactions~\citep{yang2023learningUnisim}. Moreover, actions are difficult to manipulate in these approaches and they a lot of examples of their consequences~\citep{yang2023learningUnisim}. In contrast, some recent works demonstrated that creating a physics-powered simulation of a real scenario can be effectively exploited to increase the knowledge of the robot~\citep{li2024evaluating, torne2024reconciling, abou2024physically}. However, they focus on reproducing only available observations~\citep{abou2024physically, li2024evaluating} or lack the compositional grounding to allow agents to utilize the simulation autonomously~\citep{torne2024reconciling}.\looseness=-1 

% Defintion of our manipulation world model
In this work, we demonstrate that a compositional manipulation world model can ground imagination capabilities to robots allowing the agent to exploit physically reliable predictions to increase the agent's knowledge. Thus, it is an interactable physics-constrained representation that bridges robot imagination with real world consequences. We propose to shape this grounded world model by reconstructing the scene with object-centric Gaussian Splatting~\citep{kerbl20233dgaussiansplatting} and embedding the obtained compositional scene representation into a physics simulator, e.g., PyBullet~\citep{coumans2020pybullet}. Gaussian Splatting efficiently reconstructs 3D scenes by representing them as a set of independent Gaussians that can be optimized and rendered, allowing for extremely high resolution and almost real-time graphics rendering. Its compositional characteristics are inferred using foundational models~\citep{ravi2024sam, ren2024grounded}, allowing the agent to manipulate the model to create new scenes.\looseness=-1 

% How it can be used
Through the proposed world model, it is possible to execute a robot policy directly in imagination while rendering realistic observations, a capability that can benefit imitation learning, whose objective is to solve tasks given several demonstrations. The demonstrations should contain a broad range of variations to ensure a reliable generalization of the learned policy. However, collecting data with many configurations of the environment is impractical and time-consuming in real applications~\citep{mandlekar2023mimicgen}. As shown by recent works~\citep{mandlekar2023mimicgen, pitis2022mocoda}, augmentation of the training data for imitation learning  can result in improved policies. In this work, we show that we can produce new high-quality demonstrations by imposing equivariant transformation, namely roto-translation of robot actions and objects in the scene that solve the same demonstrated task, inside the world model.
The idea is to exploit the imagination to augment the original demonstrations with generated ones, employing the proposed world model to verify that the generated actions cause the objects to reach the desired goal configuration and to render realistic observations.\looseness=-1 

% If there we can use the world model to validate models
%While our proposed world model can augment data, it can also function as a validation model. Similarly to~\citet{li2024evaluating}, we can execute the robot policy inside the simulation, but our simulation is constructed from the images of the test scenario. Consequently, we can use the world model of the robot to imagine the consequences of the actions of different policies. In this way, the robot can select the best policy based on the characteristics of the test environment.

% Summary of contributions
The contributions are: 
%(1) We develop \name: an agent equipped with an explicit, compositional, and physics-informed world model learned from RGB-D images; %compositional manipulation world model 
(1) We propose \name: a compositional manipulation world model that grounds the imagination capabilities of world models into robot manipulation;
(2) We propose to exploit the compositional structure of the learned world model to generate novel, valid, and realistic training demonstrations for imitation learning; 
%(3) We show that  \name, using a learned world model for novel data generation, is more efficient and robust in both simulated and real-world environments.\looseness=-1
(3) We demonstrate that \name improves agent generalizability even with a minimal number of demonstrations not only in simulation but also in a real setup.  \looseness=-1
% Push more on real world (not only in simulated but also in real world) and the minimal number of demonstrations (one shot maybe but to check) 


==> text/old_text/introduction_old.tex <==
\section{Introduction}
\label{sec:Introduction}
% What is a world model and why it important
In robotics, world models are learned representations of the real world that an agent can use to predict the consequences of the actions~\citep{ha2018worldmodel}. World models give robots the ability to imagine and, consequently to learn new skills~\citep{hafner2019dream, gumbsch2024learning} or new actions~\citep{pitis2020counterfactual, yang2023learningUnisim} purely in imagination. Thus, they are a fundamental building block for robots to imagine, a capability that humans exploit to correctly interact with new environments and learn new skills~\citep{Hawkins2017worldmodel, ha2018worldmodel}.

%here we say the problems they have for robotics and what they not


% What it should have
An advantageous world model should realistically represent the visual world~\citep{yang2023learningUnisim, zhou2024robodreamer}  while simulating the dynamics~\citep{li2024evaluating}, crucial for grounded and informed world reasoning. Moreover, it should allow the agent to interact with the constructed environment~\citep{yang2023learningUnisim}. 
% What are the current limitations 
One way to train a world model is to leverage internet-scale video data by fitting generative autoregressive models~\citep{yang2023learningUnisim, zhou2024robodreamer}. Whereas these models produce photo-realistic rendering, predicting the causal consequences of actions falling outside their training distribution can produce hallucinations and unrealistic interactions~\cite{yang2023learningUnisim}. In contrast, a recent work by~\citet{li2024evaluating} demonstrated that creating a physics-powered simulation of a real scenario can be effectively used as a world model to evaluate different policies. However, manually creating such representation is expensive and not scalable. 

% What we propose
In this work, we propose to learn a physics-powered compositional world model by reconstructing the scene with object-centric Gaussian Splatting, inferred using foundational models, and embedding the obtained compositional scene representation into the physics simulator. 
Gaussian Splatting~\citep{kerbl20233dgaussiansplatting} efficiently reconstructs 3D scenes by representing them as a set of independent Gaussians that can be optimized and rendered, allowing for extremely high resolution and almost real-time graphics rendering. We pair the Gaussians with dynamics engines, i.e. PyBullet~\citep{coumans2020pybullet}, to re-purpose Gaussian Splatting as a basis of embodied world models. Foundational models ensure a grouping of the Gaussians that identifies objects. Thus, they orchestrate the creation of an object-centric representation of the world. 

% How it can be used
Through a physics-powered world model, it is possible to execute a robot policy directly in imagination while rendering realistic observations, a capability that can benefit imitation learning, whose objective is to solve tasks given several demonstrations. The demonstrations should contain a broad range of variations to ensure a reliable generalization of the learned policy. However, collecting data with many configurations of the environment is impractical and time-consuming in real applications~\citep{mandlekar2023mimicgen}. As shown by recent works~\citep{mandlekar2023mimicgen, pitis2022mocoda}, augmentation of the training data for imitation learning  can result in improved policies. In this work, we show that we can produce new high-quality demonstrations by imposing equivariant transformation of the environment and the originally-collected trajectory directly inside our world model. 
The idea is to exploit the imagination to augment the original demonstrations with generated ones, exploiting the proposed world model to verify that the generated actions cause the objects to reach the desired goal configuration and to render realistic observations.

% If there we can use the world model to validate models
%While our proposed world model can augment data, it can also function as a validation model. Similarly to~\cite{li2024evaluating}, we can execute the robot policy inside the simulation, but our simulation is constructed from the images of the test scenario. Consequently, we can use the world model of the robot to imagine the consequences of the actions of different policies. In this way, the robot can select the best policy based on the characteristics of the test environment.

% Summary of contributions
The contributions are: 
(1) We develop \name: an agent equipped with an explicit, compositional, and physics-informed world model learned from RGB-D images; %compositional manipulation world model 
(2) We propose to exploit the compositional structure of the learned world model to generate novel, valid, and realistic training demonstrations for imitation learning; 
(3) We show that  \name, using a learned world model for novel data generation, is more efficient and robust in both simulated and real-world environments.\looseness=-1
% Push more on real world (not only in simulated but also in real world) and the minimal number of demonstrations (one shot maybe but to check) 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% TEXT OF THE WORKSHOP
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Humans have developed an unmatched ability to interact with their environment and can perform various tasks, such as navigation or manipulation, while using little external supervision. The crucial capability for such effective behavior is \emph{imagination}~\citep{dijkstra2023subjectiveImagina2}. 
%In robotics, learning to imagine is usually referred to as learning a world model~\cite{ha2018worldmodel}, which determines the effects of a given action on the environment to acquire new skills purely in imagination~\citep{hafner2019dream, gumbsch2024learning} and augment data by constructing new plausible robot trajectories.~\citep{pitis2020counterfactual}. 
%A useful world model shall realistically represent the visual world~\cite{yang2023learningUnisim, zhou2024robodreamer} as well as the dynamics~\cite{li2024evaluating}, both crucial for grounded and informed world reasoning.

%A useful world model has two crucial aspects: it is both visually realistic~\cite{yang2023learningUnisim, zhou2024robodreamer} and can model environment dynamics realistically~\cite{li2024evaluating}.\looseness=-1

% One way to train a world model is to leverage internet-scale video data by fitting generative autoregressive models~\cite{yang2023learningUnisim, zhou2024robodreamer}. However, autoregressive models
% % these models have a significant limitation: they 
% struggle to predict the causal consequences of actions falling outside their training distribution. As a result, such approaches can produce hallucinations and unrealistic predictions of interactions. In contrast, recent work by~\citet{li2024evaluating} demonstrated that creating a  physics-powered simulation of the real environment can be effectively used as a world model to evaluate different policies. However, manually creating such  physics-powered simulation is expensive and not scalable, thus it is crucial to study potential way to learn such  physics-powered and realistic world models from the environment observations themselves.\looseness=-1

% State-of-the-art approaches for constructing such representations leverage generative models trained on internet data~\cite{yang2023learningUnisim, zhou2024robodreamer}. However, they have a relevant limitation: they cannot easily predict causal consequences of the actions. Consequently, such approaches can be hallucinated and produce unrealistic prediction of the interaction. On the other hand, the recent work of~\citet{li2024evaluating} demonstrated that the creation of a physics-powered simulation of the real environment can be exploited for evaluating different policies. 

%Recently, Gaussian Splatting (GS)~\cite{kerbl20233dgaussiansplatting} was proposed as an efficient and effective way to reconstruct general 3D scenes. GS represents scenes through a set of independent gaussians that are quickly optimized and rendered. 
% Such ability was already exploited for creating simulation-based environment, but these focuses mainly on augmented reality~\cite{jiang2024vrgs} or creates unrealistic behavior~\cite{xie2024physgaussian}, not suitable for a \textit{world model}. 
%We noticed that the explicit representation of GS can be easily connected to standard physic  simulators, such as Bullet~\citep{coumans2015bullet}, to create an intractable representation of the scene suitable for learning robot policies.  
%Recently, Gaussian Splatting (GS)~\cite{kerbl20233dgaussiansplatting} was proposed as an efficient and effective way to reconstruct 3D scenes by representing them as a set of independent Gaussians. These can be efficiently and accurately optimized and rendered, allowing for extremely high resolution and almost real-time graphics rendering. While GS was originally proposed for inverse graphics, we observe that if we pair the Gaussians with dynamics engines, e.g. Bullet~\cite{coumans2015bullet}, we can re-purpose Gaussian Splatting to be the basics of Embodied World models. 
% In this work, we create a physics-powered world model using the GS and Bullet to create the robot imagination, demonstrating its capabilities in real applications.
%In this work, we propose to learn a physics-powered compositional world model by reconstructing the scene with object-centric GS and embedding the obtained compositional scene representation into the physics simulator. 
% Then we demonstrate flexibility of such world model for efficient imitation learning from a few demonstrations.

%Similar to humans that can imagine new realistic scenarios and learn from them, the agent can use our world model to generate new realistic training data. In particular, we consider agents in Imitation Learning (IL) that learn a task from several demonstrations. 
%By using a physics-powered world model, it is possible to execute a robot policy directly in imagination, while rendering realistic data. This capability can be exploited in Imitation Learning (IL) whose objective is to learn a task from several demonstrations.   
%To ensure a good generalization of the policy, the demonstrations should contain a broad range of variations, often impractical and time-consuming to collect in real applications~\cite{mandlekar2023mimicgen}. However, as shown by recent works~\cite{mandlekar2023mimicgen, pitis2022mocoda}, generating new training data can result in improved policies. In this work, we show that we can generate new high-quality demonstrations by imposing equivariant transformation of the environment and the originally-collected trajectory directly inside our physical simulation. 
%The idea is to exploit the world model to augment the original demonstrations with generated ones. Checking whether the generated examples can be correctly executed by the robot is also a key characteristic of the proposed  world model.

%While our proposed world model can augment data, it can also function as a validation model. Similarly to~\cite{li2024evaluating}, we can execute the robot policy inside the simulation, but our simulation is constructed from the images of the test scenario. Consequently, we can use the world model of the robot to imagine the consequences of the actions of different policies. In this way, the robot can select the best policy based on the characteristics of the test environment.
% Both the proposed demonstration augmentation and the policy validation are tested in a simulation benchmark and in a real robot experiments to prove the applicability of the proposed approaches in real applications.

% The contributions of this paper can be summarized as follows:
% \begin{itemize}
%     \item We propose a novel physics-powered and compositional world model that can be learned from RGB-D observations of the environment;
%     \item We leverage learned world model to generate new training data for IL by exploiting equivariant transformation of the demonstration trajectory and scene decomposition into objects;
%     % \item We demonstrated that by using our physics-powered world model, an agent can validate the learned policy before applying it to the real environment.
%     \item We study realism of our world model in both simulated and real-world environments, as well as usefulness of the proposed new training data generation for imitation learning.
% \end{itemize}

%%%%%%%% PROPOSED ALTERNATIVE
%The contributions are: (1) We propose a novel physics-powered and compositional world model learned from RGB-D images; (2) We propose to use physics-powered world models as an imagination engine to generate novel training trajectories for imitation learning; (3) We study the effects of the world model and the data generation in simulated and real-world environments.\looseness=-1

==> text/old_text/introduction_stratis.tex <==
\section{Introduction}
\label{sec:Introduction}

% What is a world model and why it important
World models~\citep{ha2018worldmodel}, $s_{t+1}=f_\theta(s_t, a_t, z_t)$, are dynamic representations of the world, which predict the future state of the world $s_{t+1}$ given the current state $s_t$, an action $a_t$ taken by the agent(s), and possibly a latent code $z_t$ that encodes information hidden due to partial observability.
For world models, extrapolation outside all combinations of seen states during training ---and not simply generalization between seen states--- is not merely desirable but essential for their very purpose.
For one, as we move to ever more complex and open 3D worlds \addref, it is unrealistic to expect any training distribution to encompass all possible configurations of the world.
% Thus, \emph{de facto} there will always be a domain difference between training and testing distributions, at least with arbitrarily complex and open 3D worlds \addref.
Further, if we could achieve such exhaustive coverage, we would need no more to distinguish between the agent and the world model, as there would be no novel information left to model.
Extrapolation is similar to an agent's ability to imagine beyond its direct experience.

To enable imagination beyond direct experiences, we identify three essential requirements that we need to build in as inductive biases in our world models.
First, the world model must be inherently \emph{compositional}, allowing the generation of novel and valid combinations of learned concepts.
Second, it must be \emph{object-centric}, as the world is primarily composed of objects of varying number, type, and configuration.
Third, it must be \emph{manipulable}, ensuring that actions and their consequences can be modeled in a straightforward and controllable manner.

To induce these design biases, we diverge from the recent literature~\citep{hafner2019dream,  yang2023learningUnisim, gumbsch2024learning, hansen2024tdmpc} that considers general models, and assume our world is specifically the 3D world that a robot resides.
Our world model (i) disentangles the different objects in the world, (ii) disentangles the appearance of objects from their dynamics, and uses learning only to (iii) ground appearance directly in the real-world observations of the robot.
We then pair the Gaussian Splat object representations with deterministic physics engines that precisely simulate future object states based on initial conditions and interventions.

\str{This paragraph should detail very explicitly the advantages of the disentangling and the grounding  we now have. Maybe there is more? I think this paragraph can be written better and more precisely, but I leave it for now. Perhaps there are also more benefits that I have not included. Feel free to improve it.}
Disentangling and grounding our model to the observations of the robot means that we can explicitly manipulate the objects in the world.
This level of control of the world and of the objects has several key advantages.
For one, it allows us to bridge the space of imagination with the real world observed by the robots ~\citep{abou2024physically, torne2024reconciling}.
As a consequence, the robot can anticipate the consequence of its policy before the policy is applied.
\str{Not sure if this is the best way to explain the difference with the real-world experiment of UniSim.}
Moreover, it allows us to run the learned policies near real-time without requiring conditioning on initial frames~\citep{yang2023learningUnisim}, since the modelled world is exactly the observed world as it stands.
Further, due to this level of control we are able to imagine novel robot trajectories in the real world, which we can use as imagined augmentations (or simply ``imaginations'') to increase the training set of our policy learning.
As we show experimentally, this results in significant accuracy improvements in few-shot or even zero-shot policy learning, with as little as \str{2? 4?} examples.
Last but not least, disentangling and grounding means that the learned policies are interpretable, which is important in terms of safety.

% Summary of contributions
In summary, our contributions are the following: 
%(1) We develop \name: an agent equipped with an explicit, compositional, and physics-informed world model learned from RGB-D images; %compositional manipulation world model 
(1) We propose \name: a compositional manipulation world model that grounds the imagination capabilities of world models into robot manipulation;
(2) We propose to exploit the compositional structure of the learned world model to generate novel, valid, and realistic training demonstrations for imitation learning; 
%(3) We show that  \name, using a learned world model for novel data generation, is more efficient and robust in both simulated and real-world environments.\looseness=-1
(3) We demonstrate that \name improves agent generalizability even with a minimal number of demonstrations not only in simulation but also in a real setup.  \looseness=-1
% Push more on real world (not only in simulated but also in real world) and the minimal number of demonstrations (one shot maybe but to check) 



----- END OF INTRO

\str{This goes to related work}
World models give agents the ability to observe the outcomes of actions in imagination, which is crucial for learning new skills~\citep{hafner2019dream, gumbsch2024learning, hansen2024tdmpc} or new behaviours~\citep{pitis2020counterfactual, yang2023learningUnisim}. Thus, they are a fundamental building block for robots to imagine, a capability that we humans exploit to interact with new environments and to learn new skills~\citep{Hawkins2017worldmodel, ha2018worldmodel}.\looseness=-1 

% % Explain what it is needed for a grounded world model
% Applying world models to real robots implies grounding the representation to the real scenarios in which they need to interact~\citep{yang2023learningUnisim, zhou2024robodreamer} while reliably simulating the dynamics~\citep{li2024evaluating}.
% Whereas the world model should behave realistically, the most important characteristic is its usefulness in increasing the knowledge of the robot~\citep{qureshi2024splatsim}. An agent should be capable of interacting with the model and adapting it to explore configurations out of its domain. Moreover, it should connect the real actions of the robot with actions in the world model to bridge what can be learned in imagination into reality~\citep{abou2024physically, torne2024reconciling}.\looseness=-1 

\str{This goes to related work}
% Current limitations of the apporaches 
One way to create such a world model is by learning a representation by interacting with the environment~\citep{yang2023learningUnisim, zhou2024robodreamer}. Whereas these models generalize to different objectives, predicting the causal consequences of actions falling outside their training distribution can produce hallucinations and unrealistic interactions~\citep{yang2023learningUnisim}. Moreover, actions are difficult to manipulate in these approaches and they a lot of examples of their consequences~\citep{yang2023learningUnisim}. In contrast, some recent works demonstrated that creating a physics-powered simulation of a real scenario can be effectively exploited to increase the knowledge of the robot~\citep{li2024evaluating, torne2024reconciling, abou2024physically}. However, they focus on reproducing only available observations~\citep{abou2024physically, li2024evaluating} or lack the compositional grounding to allow agents to utilize the simulation autonomously~\citep{torne2024reconciling}.\looseness=-1 


% % Defintion of our manipulation world model
% In this work, we demonstrate that a compositional manipulation world model can ground imagination capabilities to robots allowing the agent to exploit physically reliable predictions to increase the agent's knowledge. Thus, it is an interactable physics-constrained representation that bridges robot imagination with real world consequences. We propose to shape this grounded world model by reconstructing the scene with object-centric Gaussian Splatting~\citep{kerbl20233dgaussiansplatting} and embedding the obtained compositional scene representation into a physics simulator, i.e. PyBullet~\citep{coumans2020pybullet}. Gaussian Splatting efficiently reconstructs 3D scenes by representing them as a set of independent Gaussians that can be optimized and rendered, allowing for extremely high resolution and almost real-time graphics rendering. Its compositional characteristics are inferred using foundational models~\citep{ravi2024sam, ren2024grounded}, allowing the agent to manipulate the model to create new scenes.\looseness=-1 

% How it can be used
\str{Perhaps we can use some more details from here to explain in my intro how we make the augmentations.}
Through the proposed world model, it is possible to execute a robot policy directly in imagination while rendering realistic observations, a capability that can benefit imitation learning, whose objective is to solve tasks given several demonstrations. The demonstrations should contain a broad range of variations to ensure a reliable generalization of the learned policy. However, collecting data with many configurations of the environment is impractical and time-consuming in real applications~\citep{mandlekar2023mimicgen}. As shown by recent works~\citep{mandlekar2023mimicgen, pitis2022mocoda}, augmentation of the training data for imitation learning  can result in improved policies. In this work, we show that we can produce new high-quality demonstrations by imposing equivariant transformation, namely roto-translation of robot actions and objects in the scene that solve the same demonstrated task, inside the world model.
The idea is to exploit the imagination to augment the original demonstrations with generated ones, employing the proposed world model to verify that the generated actions cause the objects to reach the desired goal configuration and to render realistic observations.\looseness=-1 

% If there we can use the world model to validate models
%While our proposed world model can augment data, it can also function as a validation model. Similarly to~\citet{li2024evaluating}, we can execute the robot policy inside the simulation, but our simulation is constructed from the images of the test scenario. Consequently, we can use the world model of the robot to imagine the consequences of the actions of different policies. In this way, the robot can select the best policy based on the characteristics of the test environment.

% % Summary of contributions
% The contributions are: 
% %(1) We develop \name: an agent equipped with an explicit, compositional, and physics-informed world model learned from RGB-D images; %compositional manipulation world model 
% (1) We propose \name: a compositional manipulation world model that grounds the imagination capabilities of world models into robot manipulation;
% (2) We propose to exploit the compositional structure of the learned world model to generate novel, valid, and realistic training demonstrations for imitation learning; 
% %(3) We show that  \name, using a learned world model for novel data generation, is more efficient and robust in both simulated and real-world environments.\looseness=-1
% (3) We demonstrate that \name improves agent generalizability even with a minimal number of demonstrations not only in simulation but also in a real setup.  \looseness=-1
% % Push more on real world (not only in simulated but also in real world) and the minimal number of demonstrations (one shot maybe but to check) 


==> text/old_text/related_works_old.tex <==
\section{Related Work}
\label{sec:Related Works}

\subsection{World Models}
A world model is a representation of the environment that an agent can use to learn~\citep{ha2018worldmodel}. Humans have an abstract representation of the world suitable for predicting the consequences of actions~\citep{keller2012sensorimotor}. Such an idea is inherited by reinforcement learning to policies by imagining the consequences of the actions~\citep{ha2018worldmodel, hafner2019dream, hafner2020mastering, hafner2023mastering}. State-of-the-art approaches leverage generative models for creating world models~\citep{jia2023adriver, hu2023gaia, yang2023learningUnisim, bruce2024genie}. Recently, Genie~\citep{bruce2024genie} has been proposed as a foundational model for constructing interactive environments, deploying an 11B parameter model. While being first applied to game simulations~\citep{ha2018worldmodel, hafner2019dream} and navigation~\citep{hu2023gaia, jia2023adriver}, they have been recently applied to robotics. UniSim~\citep{yang2023learningUnisim} exploits diffusion to simulate the consequences of the robot's actions. DayDrimer~\citep{wu2023daydreamer} shows that locomotion and robot manipulation are learnable skills by using Dreamer~\citep{hafner2019dream}. 
The main problem with these approaches is the inadequacy in comprehensively capturing the consequences of motion and physics outside the training domain~\citep{yang2023learningUnisim}. This work leverages a robust simulator to create a physics-powered world model. Moreover, the proposed approach can reconstruct and simulate a realistic environment on a single machine with a mid-level GPU thanks to the recent introduction of Gaussian Splatting~\citep{kerbl20233dgaussiansplatting}.
Many works have built upon such a technique for simulating physics using particle-based simulation~\citep{xie2024physgaussian, jiang2024vrgs}. They leverage the gaussians representation as the particle representation required by the simulators.However, they often model unrealistic movements of objects since estimating the elasticity of the particles is complex. Conversely, we focused on rigid body dynamics that are more efficient to compute and could be done directly from the meshes. Recently, \citet{abou2024physically} and \citet{lou2024robo} showed the Gaussian Splatting representations can be adapted for tracking moving objects. However, they only reconstruct the scene without applying the simulation to real manipulation applications that require predictions of the novel state of the world. Instead, we show that our simulation can be effectively deployed for data generation in imitation learning, giving robots the ability to imagine. % Also policy evaluation if we have time

\subsection{Imitation learning}

Imitation learning involves collecting a dataset of demonstrations and learning a task on such data. Recently, research focused on vision-based imitation learning, where the policy is learned and executed directly from RGB or RGB-D images~\citep{zeng2021transporter, shridhar2023perceiveractor, shridhar2022cliport, goyal2024rvt2}. A significant advancement in imitation learning was Transporter~\citep{zeng2021transporter}, which introduced a network executing pick-conditioned placing. The authors analyze data augmentation, demonstrating its benefits for learning tasks but stating that imagining various object configurations is unrealistic. However, we demonstrate that generating new demonstrations is feasible thanks to recent developments in foundation models, Gaussian splatting, and physics simulation. 
%CLIPort~\cite{shridhar2022cliport} adapts Transporter for multi-task object manipulation inserting CLIP features inside the action computations, but is limited to simple pick-and-place tasks in 2D top-down settings. 
C2F-ARM~\citep{james2022coarsec2farm} and PerAct~\citep{shridhar2023perceiveractor}  voxelized the environment and inferred the action directly in 3D. RVT~\citep{goyal2023rvt}, inspired by PerAct, uses the point cloud to render images from an optimal point of view to predict the subsequent action. All these models require around one hundred demonstrations to learn a task. Recently, GNFactor~\cite{ze2023gnfactor} and RVT2~\cite{goyal2024rvt2} reduced the number of examples using  Nerf and a coarse-to-fine inference, respectively. However, they still need many examples to accurately perform a task. In this work, we show that by reconstructing a physics-powered simulation of the scene and imposing equivariant constraints on the data, we can generate new data and reduce even more the demonstrations needed.

\subsection{Data augmentation for Imitation learning}
Data augmentation is an established practice in Computer Vision. Early milestone works, such as AlexNet~\citep{krizhevsky2012imagenet} or ResNet~\citep{he2016deep}, applied random flip and crop to improve the robustness of the models. However, data augmentation in robotics poses some challenges since the robot's actions affect the environment. Thus, directly augmenting data is not always trivial.~\citet{laskin2020reinforcement} demonstrated that image augmentation, such as crop or color jitter, can help agents to learn better policies. However, their approach does not augment robot actions. Differently, our approach provides new trajectories. In MoCoDa~\citep{pitis2022mocoda},  the generation is achieved by creating counterfactual transitions between states and actions. Recently,~\citet{corradounderstanding} proposed dynamic invariant augmentations, demonstrating that expanding state-action coverage of training data is more effective than increasing transitions. 
The recently introduced MimicGen~\citep{mandlekar2023mimicgen} showed that imitation learning can benefit from data augmentation by composing different object-centric segments. The main drawback of these approaches is that they can only create data by composing known states. Conversely, we generate new data by imagining new equivariant configurations of the objects and trajectories. \citet{torne2024reconciling} propose to reconstruct the environment to fine-tune a robot policy in simulation. However, their reconstruction is manually identified and do not have the possibility to render high quality RGB-D images. Whereas we leverage foundation models to automatically extract an object-centric representation and create observations thanks to Gaussian Splatting.
%Adademo~\cite{mu2024adademo} allows to  

==> text/old_text/world_model-Sep30.tex <==
\section{Learning to Imagine with Gaussian Splatting.}
\label{sec:learning_to_imagine}
\begin{figure}
\centering
\includegraphics[width=\textwidth]{ICLR 2025 Template/images/ICLR_framework.png} \\
\caption{TODO: write caption }
\label{fig:framework}
\end{figure}

We aim to construct an object-centric interactable environment for the robot to imagine novel data that is valuable for better learning of the particular set of tasks. A \emph{compositional manipulation world model} consists of several components: a set of discovered object-centric assets in the environment $\mathcal{O} = \{o_i\}_{i=1}^N$; a model of the agent itself $\mathcal{A}$; a model of the particular manipulation tasks $\mathcal{T}$; a rendering function $f(\mathcal{O}, \mathcal{A}, \mathcal{T})$, to produce realistic observations $\mathbf{H}$ from the simulated state of all entities $\mathcal{O}$ and the agent $\mathcal{A}$. 

The manipulation world model (either implicit or explicit) should allow the execution of particular robot action sequences purely in imagination. In addition, modeling a task in the world model helps evaluate the predictions regarding a specific task (i.e., whether the action sequence solved the task or not). In the next section, we show how to construct the manipulation world model by combining an explicit object-centric 3D scene representation, the representation of the robot itself, and a physics simulator~\citep{coumans2020pybullet} while verifying the plausibility of the obtained world model dynamics using demonstration data. The proposed framework is represented in \Fig{fig:framework}.

\subsection{Object-Centric 3D Scene Decomposition}
To discover and represent accurate object assets that are embeddable into the existing physics engines, we propose to combine the zero-shot abilities of the foundational tracking model~\citep{cheng2023trackingdeva} with the photo-realism of Gaussian Splatting (GS)~\citep{kerbl20233dgaussiansplatting, huang2023went}. In this work, we assumed that objects are rigid and non-articulated. Extending manipulation world models to articulated and deformable objects is an exciting future work direction that could be tackled with Dynamic Gaussian Splatting~\citep{luiten2023dynamic}.
 
\paragraph{Scene Decomposition into Objects} Decomposing the high-dimensional scene observation into objects~\citep{Locatello2020SlotAttention, seitzer2023bridging, wu2024neural} that could be independently controllable could greatly simplify the difficulty of the control and the dynamics learning by exploiting the structure present in the environment~\citep{zadaianchuk2021selfsupervised, zadaianchuk2022self}. Given a sequence of RGB-D observations of the scene $\mathcal{I} = \left(\mathcal{I}_{\text{RGB}},\ \mathcal{I}_{\text{depth}}\right)$ collected by an agent, the objects and the table masks in the scene could be obtained using an open-vocabulary segmentation model~\citep{ren2024grounded}. To get consistent masks through the whole sequence of images $\mathcal{I}$, we use DEVA~\citep{cheng2023trackingdeva}, an open-vocabulary video segmentation model. While we use the officially released model~\footnote{\texttt{https://github.com/hkchengrex/Tracking-Anything-with-DEVA}}, the approach is flexible and can take advantage of newer zero-shot video object segmentation models, such as OV2Seg~\citep{wang2023towards} or SAM2~\citep{ravi2024sam}, without any additional modifications.
For the prompts for discovering objects, we use general and minimal prompts: \texttt{object} for all the objects and \texttt{table} for segmenting a table. First, for each object $i$, we predict its binary mask $m_i$ and then filter the original images $\mathcal{I}$ to obtain object images $\mathcal{I}_i$, keeping only the selected instance.

\paragraph{Extracting 3D Object Assets with 2D Gaussian Splatting} 
Gaussian Splatting~\citep{kerbl20233dgaussiansplatting, huang2023went} learns a photo-realistic and explicit representation of the scene that can be easily manipulated by applying roto-translation to the Gaussians' center and covariance. 

We start from object image sequence $\mathcal{I}_i$, obtained during object discovery. Object images $\mathcal{I}_i$ are used to extract and represent each object $i$ with explicit Gaussian Splatting representations $\mathcal{G}_i = \{g^1, \dots, g^{H}\}$, where each $g^j \in \mathcal{G}_i$ is a Gaussian associated with to object $i$. In particular, we used 2DGS~\citep{huang20242dgs} to extract high-quality object meshes required for embedding the objects into the physics simulator~\citep{coumans2020pybullet}. Moreover, 2DGS allows the creation of accurate renderings necessary for most of the imitation learning agents~\citep{goyal2024rvt2, shridhar2023perceiveractor, james2022coarsec2farm} by additional optimization of the depth images $d$. Each Gaussian $g \in \mathcal{G}_i$ is parameterized by the center $p = [x_p,\ y_p, \ z_p]$, the orientation $r$, scaling $s = (s_u, s_v)$, scalar $\alpha$ for the opacity and color $c$~(encoded into spherical harmonics to capture the view-dependent appearance). Unlike the original implementation of 2DGS~\citep{huang20242dgs}, we initialize the Gaussians by re-projecting the depth images using the given camera parameters. This requirement can be easily guaranteed when the camera is calibrated on the robot (see~\sec{sec:real_experiment}).  Each parameter of the Gaussians is differentiable and is supervised using object image sequence $\mathcal{I}_{i}$. The original implementation supervises only the RGB image while two regularization terms, named depth distortion and normal consistency, to align Gaussians to the surfaces. Since we have access to depth images $d_{\text{gt}} \in \mathcal{I}_{\text{depth}}$, we use them to supervise the optimization while discarding depth distortion normalization. The final loss for learning each object asset could be written as:
\begin{equation}
\mathcal{L} = \mathcal{L}_{\text{rec}} + \lambda_{\text{n}}\mathcal{L}_{\text{n}} + \lambda_{\text{depth}} \mathcal{L}_{\text{depth}}
\end{equation}
where $\mathcal{L}_{\text{rec}}$ and $\mathcal{L}_{n}$ are the reconstruction and normal losses defined in 2DGS, while  $\mathcal{L}_{\text{depth}} = \|d_{\text{gs}}-d_{\text{gt}}\|_1$ is novel depth supervision loss to penalize Gaussians with outlier's depth. The hyperparameters $\lambda_{\text{normal}}$ and $\lambda_{\text{depth}}$ are determined empirically similarly to \citet{huang20242dgs} and fixed to the same value for all experiments. 

\subsection{Embedding Learned Object Assets and Robot into the Simulator}
\label{sec:embedding_assets}
\paragraph{Objects Model} While explicit object-centric GS representations $\mathcal{G}_{i}$ are a good fit for photo-realistic rendering of the objects, they are not directly embeddable into a physics simulator as assets. Thus, one must augment the GS object representation $\mathcal{G}_{i}$ with the corresponding object mesh $M_{i}$. As we use 2DGS, the objects' meshes are extractable using TSDF, similar to the original 2DGS paper~\citep{huang20242dgs}. After this, the object mesh $M_{i} = \left( c_i, \  \rho_i,\ o_i\right)$ could be embedded into the simulator. Here $c_i$ and $\rho_i$ are mesh centers and orientations that could change through time, whereas $o_i$ are the mesh appearance parameters. In our work, objects mesh movements and their interaction with the robot are modeled by the PyBullet simulator~\citep{coumans2020pybullet}.

To construct a valid photo-realistic rendering function $f$ that reflects the changes in the state of the explicit manipulation world model, we need to update GS representation $\mathcal{G}_{i}$ if the simulator changes mesh $M_{i}$ parameters. Thus, we apply the change in mesh center $\Delta c^i$ and mesh orientation $\Delta \rho^i$ to all Gaussians $ g\in \mathcal{G}_i$ by updating their centers $p' = p + \Delta c_i$ and their orientations $r' = \Delta \rho_i \cdot r$. Normally, these transformations are only valid when the two coordinate frames (i.e., the Gaussian and PyBullet one) are aligned; otherwise, additional transformation between the two frames is needed. The alignment can be achieved using calibrated camera mounted on top of the robot (see \app{app:alignment} for more details). Thus, each discovered object in the scene is modeled as a tuple of aligned object Gaussians and object mesh $\left( \mathcal{G}_{i},\ M_{i} \right) \in \mathcal{O}$ creating objects' representation that mixes physical properties (such as gravity) and realistic rendering. 

\paragraph{Agent Model} We assume that the robot can model its own dynamics perfectly, similarly as humans have an accurate internal model~\citep{wolpert1998internal}. This assumption is reasonable for the manipulation world model, as most manipulation robots have the corresponding URDF file, allowing the instantiation of a simulator with the robot model. 
To render the robot’s appearance within the scene, we first extract the corresponding Gaussians, following the same procedure used for other objects. Specifically, we utilize the segmentation masks of the robot’s individual links to group the Gaussians. Each link’s segmentation mask helps us identify the areas that belong to the robot parts, ensuring accurate Gaussian representation for rendering purposes.
% To render the robot's appearance in the scene, we extract the Gaussians of the robot following the same procedure as for the objects, using robot's links segmentation masks to group the Gaussians. 
The Gaussians of each robot link are connected to the meshes of links of the URDF and updated correspondingly to link mesh updates.\looseness=-1
% The links' Gaussians updates are similar to other objects by shifting and rotating each Gaussian that belongs to the link mesh.


\paragraph{Model Verification from Demonstrations} 
In this work, the physical parameters are fixed. While we cannot guarantee that this approach to constructing the manipulation world model will lead to correct predictions for any action, we can still use demonstrations of tasks to verify the model’s usefulness for a specific set of tasks. Suppose the model’s predictions for replaying the sequence of actions in the demonstration result in a similar final state as the demonstration final state. In that case, the world model can be used as an interactive and compositional representation of the demonstration itself. In the next section, we show that such interactive representation allows us to augment the original demonstrations with imagined ones to train a more robust imitation learning policy. 

Physical parameter estimation is a well-known and studied topic~\citep{mehra1974optimal, chebotar2019closing, gao2022estimating, huang2023went} and some of these methods, such as ASID~\citep{memmelasid} or AdaptSim~\citep{ren2023adaptsim}, can be applied to identify them. This paper focuses on learning a photo-realistic representation of the world powered by a physics simulator and the usefulness of the manipulation world model for imitation learning. However, identifying the physical parameters of the world model is crucial for more complex tasks. Thus, we see physical parameters' identification using the given set of demonstrations as an important direction for future work. 



% \paragraph{Tasks model} A full specification of the manipulation world model should include not only realistic dynamics but also a representation of the tasks $\mathcal{T}$ to solve. In our case of goal-based tasks, the task is a function of the final state, and thus, it is solved in the imagination when the final positions of the entities are close to the desired final positions.

\subsection{Engineering the VividDreamer World Model}

% Problems encountered during the work:

% 1: We tested Gaussian grouping but the segmentation masks were noisier and the training slower.
% 2: depth rendering create noise filtered with radius removal
% 3: rendering problem when resolution is reduced causing the agent to perceive a wrong depth
% 4: Pybullet and Coppelia robot do not coinced 
% 5: Keypoints problem with the real examples
% 6: Frame alignement is important otherwise creates problems

The framework proposed to create the imagination data for imitation learning has several complex components that are interfaced. To deploy Gaussian Splatting as a key component, we encountered some unexpected challenges that we needed to solve. Here we give a brief description of some relevant problems we encountered in the development, while the Appendix gives more space to their discussion.\looseness=-1

\paragraph{Low-resolution Rendering} While Gaussian Splatting is designed for novel view synthesis, we noticed an unexpected behavior when it was deployed to render low-resolution images needed for the experiments in RLBench~\citep{james2020rlbench}. We collected $\mathcal{I}$ with dimension $1280 \times 720$ but rendered images $128 \times 128$. The change in resolution caused wrong renderings of RGB images and particularly of depth images, with wrong predictions of distances from cameras. The problem caused the robot to wrongly predict the actions. To overcome this problem, we rendered a higher-resolution image and down-sample it to the desired resolution.

\paragraph{Point Cloud Re-projection from 2D Gaussian Spatting} In the experiments, we used PerAct~\citep{shridhar2023perceiveractor} as a baseline. The model uses depth images to re-rpoject the point cloud in 3D. We noticed that the depth images rendered from the Gaussians are inaccurate along the edges of the robot and the objects. This created noisy point clouds that affected the agent. We solve it by filtering using the radius outlier removal from Open3D~\citep{zhou2018open3d}.

\paragraph{Mesh Extraction} In our approach, physics is deeply connected with the mesh since we use PyBullet as a core component. Thus, we needed to estimate high-quality meshes. The original version of Gaussian Splatting does not guarantee that Gaussians align with surfaces. Sugar~\citep{guedon2024sugar} proposes regularizations to improve mesh extraction. However, we found that Sugar' meshes are not accurate enough for reliable simulations. Thus, we use 2D Gaussian Splatting, as described in this section. 

==> text/old_text/world_model_old.tex <==
\section{Learning to Imagine and Act with Gaussian Splat}


Given a set of RGB-D observations of the scene $\mathcal{I}$ collected by an agent, we propose an approach to build a physics-powered world model exploiting the object-centric recognition ability of foundational model with the photo-realism of Gaussian Splatting and the physics-realism of PyBullet. The proposed framework is represented in Figure~\ref{}. The objects and the table in the scene are extracted using an open-vocabulary segmentation model. To give a consistent label to the set $\mathcal{I}$, the images are treated as video frames, and DEVA-tracking is used~\cite{cheng2023trackingdeva}. While the current version is used, the approach is general, and the capability of more recent models, such as SAM 2~\cite{ravi2024sam}, could be exploited without any additional requirement. Gaussian Splatting creates a photo-realistic representation of the scene that can be easily manipulated by applying roto-translation to the Gaussians' center and covariance. Movements of the objects are modeled by the PyBullet simulator~\citep{coumans2020pybullet}, creating a representation that mixes physical properties (such as gravity) and realistic rendering. The meshes make the bridge between the two, computed using 2D-GS~\cite{huang20242dgs}, an improved version of GS that can render depth images and extract high-quality meshes.
 
\subsection{Object-centric gaussians}
 
% Object filtering
We aim to create an object-centric interactable environment that the robot can use to imagine new data. The set of segmentation masks $\mathcal{M}_o$ with object instances is extracted through a foundational model, Grounded-Sam~\cite{ren2024grounded}, combined with tracking~\cite{cheng2023trackingdeva} to keep the label predicted in each frame consistent. 
We first extract each object's binary mask $M_o$ and then filter the original images, keeping only the selected instance. 
%and coloring the background to black. 
The resulting images are used to extract the gaussians splatting representations $\mathcal{G} = \{g_1, \dots, g_{H}\}$, where each $g_i$ is a gaussian. Since we want to connect gaussians with PyBullet, we used 2D-GS~\citep{huang20242dgs} to extract high-quality meshes. Moreover, 2D-GS allows to optimize depth images to create accurate renderings necessary for most of the imitation learning agents~\citep{goyal2024rvt2, shridhar2023perceiveractor, james2022coarsec2farm}. Each Gaussian $g_i$ is parameterized by the center $p_i = [x_p,y_p,z_p]$, the orientation $R_i$, scaling $S_i = (s_u, s_v)$, a scalar $op_i$ for the opacity and $c_i$ for the color, encoded into spherical harmonics to capture view-dependent appearance. Differently from the original implementation, we initialize the Guassians by re-projecting the depth images using the given parameters, a requirement that can be easily guaranteed when the camera is calibrated on the robot (\ref{sec:real_experiment}).  Each parameter of the Gaussians is differentiable~\citep{huang20242dgs} and is supervised using $\mathcal{I}$. The original implementation supervises only the RGB image while two regularization terms, named depth distortion and normal consistency, aligns Gaussians to the surfaces. Since we have access to depth images, we use them to supervise the optimization while discarding depth distortion normalization. The final loss is:
% \begin{equation}
% \mathcal{L} = \mathcal{L}_{rec} + \lambda_{n}\mathcal{L}_{n} + \lambda_{depth} \mathcal{L}_{depth}
% \end{equation}
\begin{equation}
\mathcal{L} = \mathcal{L}_{\text{rec}} + \lambda_{\text{n}}\mathcal{L}_{\text{n}} + \lambda_{\text{depth}} \mathcal{L}_{\text{depth}}
\end{equation}
where $\mathcal{L}_{\text{rec}}$ and $\mathcal{L}_{n}$ are the reconstruction and normal losses defined in 2D-GS~\cite{huang20242dgs} and  $\mathcal{L}_{\text{depth}} = \|d_{\text{gs}}-d_{\text{gt}}\|_1$ is the $\ell_1$ distance to penalize outliers. $\lambda_{normal}$ and $\lambda_{depth}$ are two hyper-parameters.The gaussians are optimized for 7000 iterations, removing black gaussians after training. The mesh is extracted using TSDF as done by 2DGS. 




\subsection{Physics-powered prediction of actions}
The table is considered a fixed object to create a surface on which the robot and the objects can interact, while the meshes of the objects are used by PyBullet~\citep{coumans2020pybullet} to simulate the physics. These are loaded into the simulator and changes applied to the mesh are propagated to the gaussians. At time $t-1$ each mesh is identified by a center $c^b_{t-1}$ and a rotation $r^b_{t-1}$. When at time $t$ forces are applied, the simulator predicts the new state of the meshes $c^b_t$ and $r^b_t$. The changes are applied to the gaussians of the corresponding objects by updating the center $p_i^t = p_i^{t-1} - c^b_{t-1} + c^b_t$ and the orientation $R_i^t = r^b_{t} \cdot ((r^b_{t-1})^{-1} \cdot R_i^{t-1})$. Normally, these transformations are only valid when the two frames, that is the Gaussian frame and the PyBullet frame, are aligned; otherwise, a transformation between the two frames is needed. However, we consider the cameras aligned, while we show that it is achievable with a calibrated camera mounted on top of the robot. 

To give the agent the ability to imagine, it needs the ability to act inside the simulation. Therefore, the robot is represented inside the world model similarly to the objects. However, the robot is an articulated object composed of links and joints. Two links are connected through a joint that has some degrees of freedom. PyBullet allows specifying the links and joints of the objects through Unified Robot Description Format (URDF) files~\citep{villasevil2024scaling}. In the current version, we consider the URDF of the robot given since producers shares such models with the CAD model, and we extract the guassians of the robot following the same procedure of the objects but using segmentation masks for each link. The guassians of each link of the robot are connected the meshes of links of the URDF. The updates of the links' gaussians follow the same procedure for simple objects.

\subsection{Imagination capabilities of the physics-powered world model}

The proposed world model has several capabilities. One of the most important is the possibility of executing robot actions inside the world model. A robot action is parametrized as a position and an orientation of the end-effector. Figure~\ref{} shows how the robot can interact with the environment, collecting observations and using them to predict the next action. Since consequences of actions, such as movements or collisions, are predicted by PyBullet, the world model allows  robots to predict causal consequences. In the subsequent section, this capability is exploited in imitation learning to execute trajectories and check that their final state is consistent with the original state. Collecting observations is a feature inherited by gaussians splatting, particularly by the gaussians representation that allows rendering realistic RGB and depth images of real scenarios. The constructed world model is a high-quality representation of the real scene in which the robot should act, named digital-twin~\citep{tao2022digital}. Consequently, generated observations in the world model are similar to real states of the world that the robot encounters during the interaction.  
The physical parameters are fixed, and the ability to replay the trajectory ensures that they are reliable. Physical parameter estimation is well known and studied topic~\cite{mehra1974optimal, chebotar2019closing, gao2022estimating, huang2023went} and some of these procedure, such as ASID~\cite{memmelasid} or AdaptSim~\cite{ren2023adaptsim}, can be applied to refine them. In this paper, we focus on learning a photo-realistic representation of the world powered by a physics simulator and on the usefulness of the explicit world model for imitation learning. The identification of the physical parameters using the given demonstrations is an important future work direction.
To summarise, our world model realistically represents the visual world and the dynamics thanks to the connection of gaussians to a physics engine. We demonstrate that such a powerful representation allows the robot to learn tasks directly in imagination. 
